The Multi-round Process Matrix

We develop an extension of the process matrix (PM) framework for correlations between quantum operations with no causal order that allows multiple rounds of information exchange for each party compatibly with the assumption of well-defined causal order of events locally. We characterise the higher-order process describing such correlations, which we name the multi-round process matrix (MPM), and formulate a notion of causal nonseparability for it that extends the one for standard PMs. We show that in the multi-round case there are novel manifestations of causal nonseparability that are not captured by a naive application of the standard PM formalism: we exhibit an instance of an operator that is both a valid PM and a valid MPM, but is causally separable in the first case and can violate causal inequalities in the second case due to the possibility of using a side channel.

==> APP3.tex <==
\section{Details for the MPM definition of causal separability\label{app:CnS}}
%
For completeness, we show explicitly that the correlations obtained through the `Born rule' \eqref{eq:MPMBorn} for MPMs can be transformed into correlations obtained with a PM extended by identity side channels. We will make use of a version of the \textit{link product} \cite{Chiribella2009}, which allows to merge combs together. In the context of our basis-independent convention for the CJ isomorphism, we define the link product between two operators $M^{CB}$ and $N^{B^*A}$, where $A$ and $C$ are separate systems or the trivial system, and $B$ and $B^*$ are mutually dual (\textit{i.e.} $\mathcal{H}^{B^*}$ and $\mathcal{H}^{B}$ are Hilbert spaces dual to each other, assuming the canonical isomorphism $(\mathcal{H}^*)^* \cong \mathcal{H}$ in the finite-dimensional case), as%
\begin{equation}\label{linkproduct}%
    \begin{gathered}%
         L^{AC} = M^{CB} \ast N^{B^* A}    : = \\
        \TrX{B B^*}{\left(M^{CB} \otimes N^{B^* A}\right) \left(\mathds{1}^{CB} \otimes Id^{BB^*}\right)},
    \end{gathered}%
\end{equation}
where $Id^{BB^*} \equiv \sum_{ij}^{d_B}  \dyad{ii}{jj}^{BB^*}$. 

Consider a quantum 2-comb $M^A\equiv M^{A_0A_1A_2A_3}$. The CP map it describes can be seen as resulting from the composition of two CP maps with an intermediate identity side channel. In the CJ representation, this is given by the link product between the corresponding 1-combs,
\begin{equation}
    M^A = M^{A_3A_2L_2} \ast Id^{L_2^*L_1^*} \ast M^{L_1A_1A_0} \quad , \label{eq:app:M^A}
\end{equation}
where $L_1^*$ is the ancillary output system of the first CP map (with CJ operator $M^{L_1A_1A_0}$), $L_2$ is the ancillary input system of the second CP map (with CJ operator $M^{A_3A_2L_2}$), and $Id^{L_2^*L_1^*}$ is the CJ operator of the identity side channel connecting these systems. 

This is explicitly given by
\begin{widetext}
\begin{equation*}
    M^A = \TrX{L_2L_2^*L_1L_1^*}{\left(M^{A_3A_2L_2} \otimes Id^{L_2^*L_1^*} \otimes  M^{L_1 A_1A_0}\right) \left(\mathds{1}^{A_3A_2} \otimes  Id^{L_2L_2^*} \otimes Id^{L_1^*L_1} \otimes \mathds{1}^{A_1A_0}\right)}.
\end{equation*}
\end{widetext}
Computing the trace over $L_2^*L_1^*$ yields
\begin{equation}\label{eq:app:LinkalaOO}
    M^A = \TrX{L_2 L_1}{\left(M^{A_3A_2L_2} \otimes M^{L_1 A_1A_0}\right) \left(\mathds{1}^{A} \otimes Id^{L_2L_1}\right)}.
\end{equation}
In this last expression, $Id^{L_2L_1} \equiv \sum_{ij}^{d_L^2} \dyad{ii}{jj}^{L_2L_1}$ is the \textit{transpose} of the CJ operator of an identity channel from $\Hilb{L_1^*}$ to $\Hilb{L_2}$ (just like a PM is the transpose of the CJ operator of a channel from the outputs of nodes to the inputs of nodes).  

Plugging equation \eqref{eq:app:LinkalaOO} into the `Born rule' between the 2-comb $M^A$ and a 2-node MPM $W$, one has 
\begin{equation}\label{eq:app:split}
    \TrX{}{M^A W} = \TrX{}{\left( M^{A_3A_2L_2} \otimes M^{L_1A_1A_0} \right) \left( W \otimes Id^{L_2L_1} \right)} ,
\end{equation}
where $ M^{A_3A_2L_2}, M^{L_1A_1A_0} $ are quantum 1-combs, and $ W \otimes Id^{L_2L_1} $ can be shown to be a valid (M)PM, hinting the formula \eqref{eq:MPMintoPM} for the general case. Indeed, formula \eqref{eq:app:M^A} can be applied repetitively in the case of a party with more than 2 nodes: $M^A = M^{{A}_{2n_A-2}{A}_{2n_A-1}{L}_{2n_A-2}} \ast\ldots    \ast M^{L_3A_3A_2L_2} \ast Id^{L_2^*L_1^*}\ast M^{{L}_{1}{A}_{1}{A}_{0}}$, and then the identity $\TrX{Y}{A^Y \cdot \TrX{X}{B^{XY}}} = \TrX{XY}{\left(\mathds{1}^X\otimes A^Y \right) B^{XY}}$ can be used to rewrite the whole expression as one overall partial trace. The tensor product being a special case of link product over the trivial system \cite{Chiribella2009}, this argument also applies to the multipartite case.

Consequently, the correlations achievable with an MPM are equivalent to those in a PM extended by side channels and we can appeal to the concept of causal separability for PMs in order to define causal separability for MPMs as it is done in Definition \ref{def:MPM_CnS}.

As shown in Ref. \cite{OG2016}, for the PM definition of causal separability, the possibility of extending the local operations of the parties to act on local ancillary input systems that may be entangled with the ancillary input systems of other parties also needs to be considered. Neglecting to do so may mistakenly lead to the conclusion that a PM is causally separable, although it is able to violate a causal inequality when using such an extension. Likewise, we have shown in the main text that neglecting the side channels lead to the same kind of problem. We end this appendix by reformulating Definition \ref{def:MPM_CnS} into one closer to Ref. \cite{OG2016,Wechs2018}, so that the consequences of local causal ordering are made explicit and extension by arbitrary ancillas and side channels is explicit.

We only need to rewrite \eqref{eq:app:split} as
\begin{equation}
    \TrX{}{M^A W} = \TrX{A_3A_2L_2}{M^{A_3A_2L_2} W_{|M^{L_1A_1A_0}}}\,,
\end{equation}
where we have defined the \textit{conditional process matrix} 
%
%
\begin{widetext}
\begin{equation}
    W_{|M^{L_1A_1A_0}} = c \;\TrX{L_1A_1A_0}{\left(  \mathds{1}^{A_3A_2L_2} \otimes M^{L_1A_1A_0} \right) (W\otimes Id^{L_2L_1})} \,.
\end{equation}
This can be shown to be a valid process matrix on the remaining node between $A_2L_2$ and $A_3$ for all the possible choices of $M^{L_1A_1A_0}$, as long as the normalisation factor is chosen such that Eq. \eqref{eq:norm} is verified. On the contrary, the analogously defined $W_{|M^{A_3A_2L_2}}$ will not always be a valid PM for all $M^{A_3A_2L_2}$ as it can lead to post-selection. This implies that when we reformulate the `Born rule' so as to make the unravelling from an $n$-node MPM to an $(n-1)$-node MPM apparent, starting the unravelling with a node that is not the first of some party is automatically forbidden. The generalisation of this unravelling procedure yields the following definition:
%
\begin{defi}[Causal separability of the MPM]\label{def:MPM_CS}
    Consider an MPM $W$ shared by $|\mathfrak{N}|$ parties. For $|\mathfrak{N}|=1$ this MPM is a deterministic quantum comb and thus causally separable. For $|\mathfrak{N}|>1$, the MPM is causally separable if and only if, for any state $\rho \in \LinOp{\bigotimes_{X\in\mathfrak{N}}\bigotimes_{i=0}^{n_X-1} \Hilb{X_{2i}'}}$ defined on an extension of the parties' input subsystems $\Hilb{X_{2i}} \rightarrow \Hilb{\tilde{X}_{2i}} = \Hilb{X_{2i}} \otimes \Hilb{X_{2i}'}$, the extended MPM can be decomposed as
    \begin{equation}
        W \otimes \rho = \sum_{X\in\mathfrak{N}} q_{\Party{X}{1}{}} W^{\rho}_{\Party{X}{1}{}}\,,
    \end{equation}
    with $q_{\Party{X}{1}{}}\geq0$, $\sum_{X\in\mathfrak{N}} q_{\Party{X}{1}{}} = 1$, and where $W^{\rho}_{\Party{X}{1}{}}$ is an MPM compatible with party $X$'s first operation being first in the causal unravelling (\textit{i.e.} there can be no signalling from the rest of the nodes to $\Party{X}{1}{}$ \cite{OG2016}), so that the conditional MPM after the first operation of $X$ has been carried out,
    \begin{equation}
        \left( W^{\rho}_{\Party{X}{1}{}}\right)_{\left|M^{X_0X'_0X_1L_1}\right.} = c \; \TrX{X_0X'_0X_1L_1}{\left( M^{X_0X'_0X_1L_1} \otimes \mathds{1} \right)\left( W^X \otimes \rho^{X'} \otimes Id^{L_2L_1} \right)} \,,
    \end{equation}
    is itself causally separable for all possible CP maps between $\LinOp{\Hilb{X_0}\otimes \Hilb{X'_0}}$ and $\LinOp{\left(\Hilb{X_1}\right)^* \otimes \left(\Hilb{L_1}\right)^*}$ represented by the CJ operator $M^{X_0X'_0X_1L_1}$. Here $L_2$ is an extension of the input system of $\Party{X}{2}{}$ and $c$ is a normalisation constant. %Subsystem $L_1$ (respectively, $L_2$) is the extension of the output system of $\Party{X}{1}{}$ (the input system of $\Party{X}{2}{}$) over which the side channel is defined.
\end{defi}
\end{widetext}

==> Version 2.0 sent to Quantum/APP1.tex <==
\section{Projective formulation}
%
\subsection{The projective superoperator \label{app:projo}}
%
This section aims to introduce the reader to the mapping $ \Dep{X}{} : \LinOp{\Hilb{}} \rightarrow \LinOp{\Hilb{}}$, defined as
\begin{equation}
    \DepPar{X}{\cdot} = \MapX{X}{\cdot} \,, \label{eq:Depolop}
\end{equation}
where $X$ is a tensor factor of $\Hilb{}$, and $d_X$ its dimension. It was introduced in Ref. \cite{Witness} alongside its shorthand prescript notation. To illustrate its properties, we consider an operator $M$ defined on some space $\LinOp{\Hilb{A} \otimes \Hilb{B} \otimes \Hilb{C}}$ of dimension $d^2 = (d_A d_B d_C)^2$. 

We define a multiplication within the prescript that corresponds formally to a composition of several maps as
\begin{equation}
	\MapX{A}{\MapX{B}{M}} \equiv \Dep{AB}{M} \,.
\end{equation}
This \enquote{multiplication} inherits the properties of partial tracing: it possesses an identity element (see below), it is associative as well as commutative as partial tracings on different subsystems are associative and commute, but it does not possess an inverse. Next, note that this mapping is CPTP, as well as idempotent: 
\begin{equation}\label{eq:app:idempot}
	\Dep{AA}{M} = \Dep{A^2}{M} = \Dep{A}{M} \,.
\end{equation}
    
Using the Hilbert-Schmidt product as the inner product on the space of linear operators,
\begin{gather}
	\InProd{\cdot}{\cdot} \,:\, \LinOp{\Hilb{}} \times \LinOp{\Hilb{}} \rightarrow \mathbb{C} \quad , \notag \\
	M,N \mapsto \InProd{M}{N} \equiv \TrX{}{M^\dag \cdot N}\quad,
\end{gather}
one can verify that the mapping is self-adjoint with respect to it. Let $N \in \LinOp{\Hilb{A} \otimes \Hilb{B} \otimes \Hilb{C}}$ be another arbitrary operator defined on the same space as $M$, then
\begin{align}
	\InProd{M}{\Dep{A}{N}} &=\TrX{ABC}{M^\dag \cdot \left( \MapX{A}{N} \right)} \notag \\
	&= \TrX{BC}{ \TrX{A}{M^\dag} \cdot \frac{1}{d_A}\,\TrX{A}{N}} \notag \\
	&= \TrX{ABC}{\left( \MapX{A}{M^\dag} \right) \cdot N}\, ,
\end{align}
where the identity $ \TrX{ABC}{ U^{ABC}\cdot \left(\mathds{1}^A \otimes V^{BC}\right) } = \TrX{BC}{\TrX{A}{U^{ABC}} \cdot V^{BC} }$ have been used to go to the second and third lines.
Thus,
\begin{equation}\label{eq:app:selfadj}
	\InProd{M}{ \Dep{A}{N} } = \InProd{ \Dep{A}{M} }{N}\quad.
\end{equation}
This means that the mapping is idempotent and self-adjoint, making it an orthogonal projector onto a subspace of $\LinOp{\Hilb{A} \otimes \Hilb{B} \otimes \Hilb{C}}$.

We define a linear addition operation within the prescript as 
\begin{equation}
	\Dep{A}{M} + \Dep{B}{M} \equiv \Dep{ A + B}{M} \,,
\end{equation}
and for each element $\DepPar{A}{\cdot}$ we define the inverse element $\DepPar{-A}{\cdot} \equiv - \MapX{A}{\cdot}$, such that $\Dep{A+(-A)}{M} \equiv \Dep{0}{M} = 0$, where $\Dep{0}{}$ is the additive identity element, which corresponds to the zero mapping. We will introduce the minus sign as a shorthand notation $\Dep{A+(-A)}{M} \equiv \Dep{A-A}{M}$ for addition of inverse elements. With this addition and multiplication, the prescripts have the algebraic structure of a ring \cite{herstein1975topics}. One could also promote the structure to an algebra by defining a scalar multiplication the same way the inverse additive element have been defined, \textit{i.e.} $\DepPar{\lambda A}{\cdot} \equiv \lambda\MapX{A}{\cdot}$, for all $\lambda \in \mathbb{C}$. However, note that the idempotency property is not in general conserved under scalar multiplication nor under addition of prescripts. Hence, for the purposes of this article, we restrict the algebra to a ring and we only consider combinations under addition that result in valid projectors, \textit{i.e.} idempotent elements. 

Finally, we define 2 particular elements of the ring. One is the identity mapping $\mathcal{I}$, such that $\mathcal{I}[M] = M$ for all operators, which corresponds to the multiplicative identity element in the ring. In prescript notation it is then denoted as a 1:
\begin{equation}
    \mathcal{I}[M] \equiv \Dep{1}{M}\,.
\end{equation}
The other is the multiplicative absorbing element $\mathcal{D}: \mathcal{D}\Proj{}{} = \Proj{}{}\mathcal{D} = \mathcal{D}$, for every $\Proj{}{}$ in the ring, which is no other than the projector to the subspace spanned by the unit matrix $\frac{1}{d}\mathds{1}$, or equivalently the mapping applied on the full system $\mathcal{D}(M) = \MapX{}{M}$. In our example, $\mathcal{D}$ is written in prescript notation as
\begin{equation}
    \mathcal{D}[M] \equiv \Dep{ABC}{M} \,.
\end{equation}
We will also use superscripts when those projectors are applied on parts of composite subsystems, \textit{e.g.} $\left(\mathcal{I}^A\otimes \mathcal{D}^{BC}\right)[M] \equiv \Dep{1BC}{M} = \Dep{BC}{M}$.
%
\subsection{Comb conditions in projective formulation \label{app:CombCd}}
%
In this section, we derive an alternative formulation of the set of necessary and sufficient constraints an operator has to satisfy to be a valid deterministic quantum comb (Eqs. \eqref{eq:QuComb_Chiri}, see \cite[Theorems 3 and 5]{Chiribella2009}). This formulation is in the spirit of what was done in Ref. \cite{Witness} for the PM validity conditions. We will find a recursive way of building the projector onto the subspace of valid quantum combs for an increasing number of teeth. To do so, we use the shorthand notation $M^{(j)} \equiv M^{X_0X_1\cdots X_{2j-1}}$, so that $M^X \equiv M^{(n_X)}$, to refer to a deterministic quantum comb with $j$ teeth. %Note that we will often write `comb' instead of `deterministic quantum comb' to lessen clutter.

The set of conditions to be proven equivalent to \eqref{eq:QuComb_Chiri} are equations \eqref{eq:QuComb} and \eqref{eq:ProjComb}, rewritten here for convenience:%
\begin{subequations}
    \begin{gather}
        M^X\geq0 \,,\label{eq:app:QuComb_positivity}\\
        \mathcal{P}_{n_X}^{X}\left[M^X\right] = M^X \,,\label{eq:app:QuComb_subspace}\\
        \TrX{}{M^X} = \prod_{j=0}^{n_X-1} d_{X_{2j}} \,,\label{eq:app:QuComb_normalisation}
        %\mathcal{D}\left(M^X\right)=\frac{\mathds{1}^{X_0X_1...X_{2n_X-1}}}{\prod_{i=0}^{2n_X-1} d_{X_{2i+1}}}
    \end{gather}%
    \label{eq:app:QuComb}%
\end{subequations}%
where $\mathcal{P}_{n_X}^{X}\equiv \mathcal{P}_{n_X}^{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X}{}} $ is the projector to the validity subspace of $n_X$-combs, which is given by the recursive relation \eqref{eq:ProjComb}
\begin{equation}\label{eq:PC}
    \begin{split}
        &\mathcal{P}_{0} = \DepPar{1}{\cdot} \,,\\
        &\mathcal{P}_{n_X}^{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}\prec \Party{X}{n_X}{}} =\\
        &\,\DepPar{\left(1-X_{2n_X-1}\right)}{\cdot} + \DepPar{X_{2n_X-2}X_{2n_X-1}}{\Proj{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}}{n_X-1}} .
    \end{split}
\end{equation}
Keep in mind that we are using the shorthand notation $\Proj{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}}{n_X-1} \equiv \Proj{X_0\ldots X_{2n_X-3}}{n_X-1} \otimes \mathcal{I}^{X_{2n_X-2}X_{2n_X-1}}$ to indicate that we are projecting the subsystems $X_0\ldots X_{2n_X-3}$ on a subspace of quantum ($n_X$-1)-combs with causal ordering $\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}$.

Note that condition \eqref{eq:app:QuComb_positivity} is just condition \eqref{eq:QuComb_Chiri_pos}---the condition that a quantum comb is PSD, which reflects the fact that it is the CJ operator of a CP map. Therefore, equivalence between the set of conditions \eqref{eq:QuComb_Chiri} and the set of conditions \eqref{eq:app:QuComb} with \eqref{eq:PC} would follow if we show that \eqref{eq:QuComb_Chiri_subspace} is equivalent to \eqref{eq:app:QuComb_subspace} and \eqref{eq:app:QuComb_normalisation}, with the projector in \eqref{eq:app:QuComb_subspace} given by \eqref{eq:PC}. This is what we show next.

The normalisation condition \eqref{eq:app:QuComb_normalisation} for deterministic combs is obtained directly by taking the total trace of the comb. We can indeed use the identity $\TrX{AB}{M^A \otimes N^B} = \TrX{A}{M^A} \TrX{B}{N^B}$, which allows to nest the set of linear constraints \eqref{eq:QuComb_Chiri_subspace} within one another. As it yields $\TrX{X_{2i-1}X_{2i-2}}{M^{(i)}} = d_{X_{2i-2}} \; M^{(i-1)}$, one can see that the total trace of a valid comb is equal to the product of its input dimensions (reflecting the fact that a deterministic quantum comb correspond to a channel from all inputs to all outputs). Hence, Eq. \eqref{eq:app:QuComb_normalisation} is a necessary condition.

%Equivalently, the map $\mathcal{D} := \frac{\mathds{1}^X}{d_X}\TrX{X}{\cdot}$ is giving the normalisation condition as
%\begin{equation}\tag{\ref{eq:app:QuComb_normalisation}}
%    \mathcal{D}\left(M^X\right)=\frac{\mathds{1}^{X_0X_1 \ldots X_{2n_X-1}}}{\prod_{i=0}^{2N_X-1} d_{X_{2i+1}}}
%\end{equation}

We next show that for a 1-comb, Eq. \eqref{eq:app:QuComb_subspace} with the projector $\Proj{X}{1}$ defined as in \eqref{eq:PC} is necessary. Indeed, the constraint for a 1-comb is equivalent to
\begin{align}
    \TrX{X_1}{M^{(1)}}\,&=\,\mathds{1}^{X_0} & \iff \nonumber\\
    %\frac{\mathds{1}^{X_1}}{d_{X_1}}\otimes\TrX{X_1}{M^{(1)}}\,&=\,\frac{\mathds{1}^{X_0X_1}}{d_{X_1}} &\iff \\
    \Dep{X_1}{M^{(1)}} &= \frac{\mathds{1}^{X_0X_1}}{d_{X_0}d_{X_1}} \; d_{X_0}& \overset{\eqref{eq:app:QuComb_normalisation}}{\Longrightarrow} \nonumber\\
    \Dep{X_1}{M^{(1)}} &= \Dep{X_0X_1}{M^{(1)}} &, \label{eq:app:P^1_raw}
\end{align}
where we multiplied by $\frac{\mathds{1}^{X_1}}{d_{X_1}} \otimes$ on both sides between the first and second lines, and we used the definition \eqref{eq:Depolop} on the left-hand side, then we used Eq. \eqref{eq:app:QuComb_normalisation}, \textit{i.e.} $\TrX{}{M^{(1)}}=d_{X_0}$, together with \eqref{eq:Depolop} on the right-hand side to go to from the second line to the last. Hence, \eqref{eq:app:P^1_raw} is necessary.

The relation \eqref{eq:app:P^1_raw} is rephrased as a projector as $M^{(1)} - \Dep{X_1}{M^{(1)}} + \Dep{X_0X_1}{M^{(1)}} = M^{(1)}$ \cite{Dynamics}, or
\begin{equation}\label{eq:app:P^1}
    \Proj{X}{1}\left[M^{(1)}\right] \equiv \Dep{1-X_1+X_0X_1}{M^{(1)}} = M^{(1)} \,,
\end{equation}
where we have defined the 1-comb projector $\Proj{X}{1} \equiv \Proj{\Party{X}{1}{}}{1}$ from the space of operators $\LinOp{\Hilb{X_0}\otimes \left(\Hilb{X_1}\right)^*}$ to the subspace of (nonnormalised) deterministic quantum 1-combs. It is a projector as the relation $\left( 1-X_1+X_0X_1 \right)^2 = 1-X_1+X_0X_1$ follows from the algebraic rules of the ring defined in Sec. \ref{app:projo}. This last equation, \eqref{eq:app:P^1}, is exactly \eqref{eq:app:QuComb_subspace} with \eqref{eq:PC} in the case of 1-combs, proving their necessity in this case. 

To prove that Eqs. \eqref{eq:app:QuComb_subspace} and \eqref{eq:app:QuComb_normalisation} with \eqref{eq:PC} are sufficient to enforce Eqs. \eqref{eq:QuComb_Chiri_subspace} in the 1-comb case, we start from the projective condition,
\begin{multline}
	%\begin{aligned}
    \Dep{X_1}{M^{(1)}} - \Dep{X_0X_1}{M^{(1)}} = 0  \\
    \iff \\
    \frac{\mathds{1}^{X_1}}{d_{X_1}} \otimes \left(\TrX{X_1}{M^{(1)}}-\TrX{X_1}{\Dep{X_0}{M^{(1)}}}\right) =0 \\
    \iff \\
    \TrX{X_1}{M^{(1)}}-\frac{\mathds{1}^{X_0}}{d_{X_0}}\TrX{X_0X_1}{{M^{(1)}}} =0  \\
    \overset{\eqref{eq:app:QuComb_normalisation}}{\Longrightarrow} \\
    \TrX{X_1}{M^{(1)}} - \mathds{1}^{X_0} = 0 \, ,
	%\end{aligned}
\end{multline}

where we successively used the fact that prescripts commute and the distributive property of the tensor product to go to the second line, and \eqref{eq:Depolop} to make the full trace appear in the third line. Injecting \eqref{eq:app:QuComb_normalisation} we reach \eqref{eq:QuComb_Chiri_subspace} in the last line. Therefore,  \eqref{eq:app:QuComb_subspace} and \eqref{eq:app:QuComb_normalisation} with \eqref{eq:PC} imply \eqref{eq:QuComb_Chiri_subspace} for the case of 1-combs. This completes the proof of equivalence in this case. %\[\TrX{X_1}{M^{(1)}}=\mathds{1}^{X_0} \iff \Dep{X_1}{M^{(1)}} = \Dep{X_0X_1}{M^{(1)}}\,.\]%

Equivalence in the general case as well as a rule for building the $n_X$-comb projector can be proven by induction. Suppose that the reformulation holds up to $n_X-1$ teeth such that, for $2\leq j \leq n_X-1$,
\begin{equation}\label{eq:app:P^nX-1}
    \begin{gathered}
        \TrX{X_{2j-1}}{M^{(j)}} = \mathds{1}^{X_{2j-2}} \otimes M^{(j-1)},\\
        \TrX{X_1}{M^{(1)}} = \mathds{1}^{X_0}\,,\\
        \iff \\
        \Proj{X}{n_X-1}\left[M^{(n_X-1)}\right] = M^{(n_X-1)} \,, \\
        \TrX{}{M^{(n_X-1)}} = \prod_{j=0}^{n_X-2} d_{X_{2j}} \,,
    \end{gathered}
\end{equation}
where $\Proj{X}{n_X-1} \equiv \mathcal{P}_{n_X}^{\Party{X}{1}{}\prec \Party{X}{2}{} \prec \ldots \prec \Party{X}{n_X-1}{}}$ is the $(n_X-1)$-comb projector. To prove that the $n_X$ case of \eqref{eq:app:QuComb} follows from \eqref{eq:QuComb_Chiri}, we start with $\TrX{X_{2n_X-1}}{M^{(n_X)}} =  \mathds{1}^{X_{2n_X-2}} \otimes M^{(n_X-1)}$. We already know that the trace condition will be satisfied, so to find the projective condition we write
\begin{multline}
%\begin{aligned}
    \TrX{X_{2n_X-1}}{M^{(n_X)}} =  \mathds{1}^{X_{2n_X-2}} \otimes M^{(n_X-1)} \, ,\\
    \Dep{X_{2n_X-1}}{M^{(n_X)}} =  \frac{\mathds{1}^{X_{2n_X-2}X_{2n_X-1}}}{d_{X_{2n_X-1}}}\otimes M^{(n_X-1)} \, ,\\
    \Dep{X_{2n_X-1}X_{2n_X-2}}{M^{(n_X)}} = \frac{\mathds{1}^{X_{2n_X-2}X_{2n_X-1}}}{d_{X_{2n_X-1}}} \otimes M^{(n_X-1)}  \, ,\\
    \DepPar{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}} = \\
     \frac{\mathds{1}^{X_{2n_X-2}X_{2n_X-1}}}{d_{X_{2n_X-1}}} \otimes M^{(n_X-1)}  \, ,
%\end{aligned}
\end{multline}
where we applied successively $\frac{\mathds{1}^{X_{2n_X-1}}}{d_{X_{2n_X-1}}}\otimes $, $\DepPar{X_{2n_X-2}}{\cdot}$, and $\ProjOn{X}{n_X-1}{\cdot}$ on both sides to show that equivalence in the $n_X-1$ case implies the following relation in the $n_X$ case:%
\begin{multline}
    \TrX{X_{2n_X-1}}{M^{(n_X)}} =  \mathds{1}^{X_{2n_X-2}} \otimes M^{(n_X-1)} 	\Longrightarrow \\
    \Dep{X_{2n_X-1}}{M^{(n_X)}} = \DepPar{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}}.
\end{multline}
This last relation is actually the recursive definition $\eqref{eq:PC}$ of the projector as it can be rephrased as
%The projector is indeed built from $\Dep{X_{2n_X-1}}{M^{(n_X)}} = \DepPar{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}}$ as
\begin{equation}
    \begin{split}
        &M^{(n_X)} - \Dep{X_{2n_X-1}}{M^{(n_X)}} \\
        &+ \DepPar{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}} = M^{(n_X)}\,,\\
        &\equiv \ProjOn{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}\prec \Party{X}{n_X}{}}{n_X}{M^{(n_X)} }= M^{(n_X)} \,.
    \end{split}
\end{equation}
This yields the definition \eqref{eq:PC}.

To prove that this relation indeed defines a projector, notice the pattern in the prescripts of the recursive relation: let $\mathcal{P}_{n_X}^{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}\prec \Party{X}{n_X}{}} =  1 - B + ABC $, where $A \equiv \Dep{X_{2n_X-2}}{}$ and $B \equiv \Dep{X_{2n_X-1}}{} $ are idempotent elements, while $C \equiv \Proj{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}}{n_X-1}$. In the case $n_X=1$, $\Dep{C}{} =1$, which is idempotent, in the case $n_X=2$, $\Dep{C}{} = \Proj{\Party{X}{1}{}}{1}$, which has been proven idempotent as well. If we assume $C$ to be idempotent up to $n_X-1$, then for $n_X$:
\begin{equation}
\begin{aligned}
    \left( 1-B+ABC \right)^2 =& \left(1-B\right)^2 + 2 \left(1-B\right)ABC\\
     & \, + \left(ABC \right)^2 \\
    %=& \left(1-B\right)^2 + 2 A\left(B-B^2\right)C + A^2B^2C^2\\
    %=& (1-2B+B^2) + A0C + ABC\\
    =& 1-B + 0 + ABC \, ,
\end{aligned}
\end{equation}
where we have used the distributive property of multiplication as well as idempotency of all elements to show that $1-B + ABC$ is idempotent as well. This proves that the objects built in equation \eqref{eq:PC} are idempotent for all $n_X$, thus they define projectors.

Hence, by induction we have that conditions \eqref{eq:app:QuComb} with \eqref{eq:PC} are necessary for \eqref{eq:QuComb_Chiri}. Sufficiency is also proven by induction. Suppose \eqref{eq:app:P^nX-1} holds. For the $n_X$ case we have the implication
\begin{multline}
    \ProjOn{\Party{X}{1}{}\prec \ldots \prec \Party{X}{n_X-1}{}\prec \Party{X}{n_X}{}}{n_X}{M^{(n_X)} }= M^{(n_X)}\\
    \iff\\
    \Dep{X_{2n_X-1}}{M^{(n_X)}} - \DepPar{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}} =0 \\
    \Longrightarrow \\
    \TrX{X_{2n_X-1}}{M^{(n_X)} - \DepPar{X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}}} =0 ,
\end{multline}
yielding 
\begin{multline} 
\TrX{X_{2n_X-1}}{M^{(n_X)}} =\\
 \frac{\mathds{1}^{X_{2n_X-2}}}{d_{X_{2n_X-2}}} \otimes \TrX{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}}\,.
\end{multline}%
Because of equations \eqref{eq:app:P^nX-1}, we must have that%
\begin{equation}
	\TrX{X_{2n_X-1}X_{2n_X-2}}{\ProjOn{X}{n_X-1}{M^{(n_X)}}} \propto M^{(n_X-1)}.
\end{equation}%
Tracing out both sides, we find that the proportionality constant has to be equal to $d_{X_{2n_X-2}}$ in order for condition \eqref{eq:app:QuComb_normalisation} to hold. Thus, $\TrX{X_{2n_X-1}}{M^{(n_X)}} =  \mathds{1}^{X_{2n_X-2}} \otimes M^{(n_X-1)}$ follows from \eqref{eq:app:QuComb}. Adding this condition to the $n_X-1$ other conditions $\TrX{X_{2j-1}}{M^{(j)}} = \mathds{1}^{X_{2j-2}} \otimes M^{(j-1)}$, $2\leq j \leq n_X-1$ and $\TrX{X_1}{M^{(1)}} = \mathds{1}^{X_0}$, that were already assumed in Eqs. \eqref{eq:app:P^nX-1}, gives the $n_X$ conditions \eqref{eq:QuComb_Chiri_subspace} for an deterministic quantum $n_X$-comb. Hence \eqref{eq:app:QuComb} with \eqref{eq:PC} implies \eqref{eq:QuComb_Chiri} by induction, proving sufficiency.

Note that Eq. \eqref{eq:PC} admits an \enquote{unravelled} formulation,
\begin{equation}\label{eq:PCunravelled}
    \Proj{X}{n_X} = \DepPar{\left( 1-X_{2n_X-1} \left( 1-X_{2n_X-2}  \big( \ldots \big( 1-X_{1} \big( 1-X_{0} \big) \big) \ldots \big) \right) \right)}{\cdot} \,,
\end{equation}
shortened in 
\begin{equation}
	\Proj{X}{n_X} = \mathcal{I} - \DepPar{X_{2n_X-1}}{ \mathcal{I}-\DepPar{X_{2n_X-2}}{ \Proj{X}{n_X-1} } } \,.
\end{equation}%
This will be useful in the proof of Theorem \ref{theo:complement} presented in the next section.

\section{Proof of Theorem \ref{theo:complement} \label{app:Complement}} 
As \eqref{eq:MPM_pos} is the same condition as \eqref{eq:pos}, the proof consists in showing that condition \eqref{eq:MPM_norm} is equivalent to conditions \eqref{eq:complProj} and \eqref{eq:norm}. %In this section we will refer to an arbitrary tensor product of deterministic combs as $M \equiv \bigotimes_{X\in\mathfrak{N}} M^X$.
%We also pointed out in the main text that condition \eqref{eq:MPM_norm} is equivalent to \eqref{eq:MPM_norm_affine}. Thus, Theorem \ref{theo:complement} is proven here by showing that condition \eqref{eq:MPM_norm_affine} is verified if and only if conditions \eqref{eq:complProj} and \eqref{eq:norm} are verified.


%The tensor product of the valid deterministic combs to be plugged in the MPM $W$ are PSD operators that belong to the set \[\{M\} \equiv \left\{M \in \LinOp{\Hilb{}} | M \geq 0 , \ProjOn{}{}{M}=M , \TrX{}{M} = d_{in} \right\},\] where $\mathcal{P} \equiv \left(\bigotimes_{X \in \mathfrak{N}} \Proj{X}{n_X}\right)$, and $d_{in}\equiv \prod_{X\in\mathfrak{N}} d_{X_{in}}$. The theorem aims to characterise the set $\{W\}$ of PSD operators normalised on this set. Note that in this appendix the object to be plugged in $W$ is denoted by $M$ but can be in general the tensor product of $|\mathfrak{N}|$ different combs, each corresponding to a different party. %Indeed, a tensor product of combs belongs to a set with an algebraic structure similar as the one of a single comb \eqref{eq:QuComb}, the resulting overall projector on the full space being the tensor product of each projector on the valid comb subspace associated with a single party, \textit{e.g.} $\Proj{A B}{n_A+n_B} \equiv \Proj{A}{n_A} \otimes \Proj{B}{n_B}$ for the overall projector on the subspace of operators that are linear sums of tensor product composition of $A$'s and $B$'s combs where $A$ cannot signal to $B$ and vice-versa (see Fig. \ref{fig:CombCompo}, leftmost case). 
%For the discussion that will ensue we will work as if there was a single overall party $X$ referring to the full system, regardless of how it is split into several subsystems distributed among between any number of parties. This follows from the observation that $\{M\}$ have the same algebraic structure as the one of single deterministic quantum combs, Eqs. \eqref{eq:QuComb}.

The first step of the proof is to notice that since $\frac{\bigotimes_{X \in \mathfrak{N}} \mathds{1}^X}{\prod_{X\in\mathfrak{N}}\prod_{i=0}^{n_X-1} d_{X_{2i+1}}} \equiv \frac{\mathds{1}}{ d_{out}}$ is a valid tensor product of deterministic quantum combs, the normalisation \eqref{eq:MPM_norm} implies that the set $\{W\}$ have fixed trace norm,
\begin{equation}\label{eq:app:W_norm}
    \TrX{}{W\cdot \frac{\mathds{1}}{d_{out}}} = 1 \iff \TrX{}{W} =  d_{out} \,.
\end{equation}
%where $d_{out}\equiv \prod_{X\in\mathfrak{N}} d_{X_{in}} \equiv \prod_{X\in\mathfrak{N}}\prod_{i=0}^{n_X-1} d_{X_{2i}}$. 
This is condition \eqref{eq:norm}, which is thus necessary. It also implies that $W=\frac{\bigotimes_{X \in \mathfrak{N}} \mathds{1}^X}{\prod_{X\in\mathfrak{N}}\prod_{i=0}^{n_X-1} d_{X_{2i}}} \equiv \frac{\mathds{1}}{d_{in}}$ is an element of the set of valid MPMs since $\TrX{}{\frac{\mathds{1}}{ d_{in}}\cdot \bigotimes_{X\in\mathfrak{N}} M^X} = 1$ for all $M^X$. This actually corresponds to enforcing condition \eqref{eq:QuComb_norm} on each comb in the tensor product.

For proving the necessity of \eqref{eq:complProj} (and subsequently its sufficiency together with \eqref{eq:norm}), we will work in a convenient Hilbert-Schmidt (HS) basis $\{\sigma_i\}$ for an operator space of dimension $d^2$, whose elements satisfy
\begin{equation}\label{eq:HSbasis}
 \begin{gathered}
    \sigma_i^\dag = \sigma_i \, , \forall i \, ,\\
    \sigma_0 = \mathds{1}\, ,\\
    \TrX{}{\sigma_i} = 0 \, , \forall i \neq 0\, ,\\
    \TrX{}{\sigma_i \cdot \sigma_j} = d \, \delta_{i,j}\, ,\, \forall i,j\,,
\end{gathered} 
\end{equation}
where $\delta_{i,j}$ is the Kronecker delta.

An arbitrary operator $O\in \LinOp{\Hilb{X_0} \otimes \Hilb{X_1} \otimes \ldots}$ can always be expressed in a product basis of the kind described above: $O=\sum_{i_{0},i_{1}\ldots} o_{i_{0},i_{1}\ldots} \; \GGB{X_0}{i_{0}}\otimes \GGB{X_1}{i_{1}} \otimes \cdots$, where $\sigma_j^Y$ is the $j$-th element of a basis of subsystem $Y$ that respects \eqref{eq:HSbasis}, while the $o_{i_{0}i_{1}\ldots} \in \mathbb{C} \,, \forall i_0, \forall i_1,\ldots$ are the associated coefficients of the basis expansion, and the sum runs over all indices: $\sum_{i_{0},i_{1}\ldots} \equiv \sum_{i_0=0}^{d_{X_0}^2-1}\sum_{i_1=0}^{d_{X_1}^2-1}\cdots$. Let $\mathbf{i}=(i_{0},i_{1},\ldots)$ be a multi-index, ranging from 0 to $d_X^2-1$, with first element $\mathbf{0}\equiv (0,0,\ldots) $. Each sub-index corresponds to a subsystem  of X, \textit{i.e.} $i_0$ refers to the index of the $X_0$ component, $i_1$ to the one of $X_1$, etc... We use it to shorten the basis expansion: %
\begin{equation}
O=\sum_{i_{0}i_{1}\ldots} o_{i_{0}i_{1}\ldots} \; \GGB{X_0}{i_0}\otimes \GGB{X_1}{i_1} \otimes \ldots \equiv \sum_{\mathbf{i}} o_{\mathbf{i}} \; \GGB{X}{\mathbf{i}}\,.
\end{equation}

The action of the mapping \eqref{eq:Depolop} defined in section \ref{app:projo} on an operator is to remove certain terms in the basis expansion, as it is projecting on a subset of the basis elements of this type of basis. One can see it as if the superoperator was setting its corresponding sub-index in the HS basis to 0: $\Dep{X_0}{O}= \sum_{\mathbf{i}=(i_0=0,i_1,i_2,\ldots)} o_{\mathbf{i}} \; \GGB{X}{\mathbf{i}}$; the notation under the sum is to be understood as \enquote{summing only over all $\mathbf{i}$ for which $i_0=0$}. For example, $\DepPar{X_0}{\sum_{i_0} o_{i_0} \; \GGB{X_0}{i_0}} = o_{0} \; \GGB{X_0}{0}$, $\DepPar{X_0}{\sum_{i_0i_1} o_{i_0 i_1} \; \GGB{X_0}{i_0} \otimes \GGB{X_1}{i_1}} = \sum_{i_1} o_{0i_1} \; \GGB{X_0}{0} \otimes \GGB{X_1}{i_1}$, etc...
%$\Dep{X_1}{O}= \sum_{\mathbf{i}=(i_0,0,i_2,\ldots)} o_{\mathbf{i}} \; \GGB{X}{\mathbf{i}}$; ... 

Actually, the projector on the comb validity subspace also shares this property, and so does any tensor product of several projectors of this kind (\textit{i.e.} the projector on $\mathrm{Span}\left\{\bigotimes M\right\}$). This is the content of the following lemma.
\begin{lemm} \label{lemm:P=remover}
    The (tensor product of) mapping(s) $\Proj{X}{n_X}$ defined as in Eq. \eqref{eq:PC} is a superoperator projector whose action is to remove certain basis elements in the Hilbert-Schmidt expansion of an arbitrary CJ operator.
\end{lemm}
\begin{proof}
    The proof is based on the following two observations: (a) Let $\Proj{}{}$ be a projector whose action in the HS basis expansion amounts to removing certain types of terms while leaving the others intact. Then, $\mathcal{I} - \Proj{}{}$ is a projector that also has this property. Indeed, it will leave the terms that are removed by $\Proj{}{}$ and will remove those that are left by $\Proj{}{}$.
    (b) Let $\Proj{}{}$ and $\Proj{'}{}$ be two projectors whose action in the basis expansion amounts to removing certain types of terms. Then the product $\Proj{'}{}\Proj{}{}$ is also a projector of this kind. Indeed, $\Proj{}{}$ would first remove the terms it removes, and then $\Proj{'}{}$ would remove those that it removes from what remains after the action of $\Proj{}{}$. Note that this observation implies in particular that if the claimed property holds for $\Proj{X}{}$ and $\Proj{'Y}{}$ that act on separate systems, it also holds for their tensor product $\left(\Proj{X}{}\otimes \mathcal{I}^Y\right)\left(\mathcal{I}^X \otimes \Proj{'Y}{}\right)$, since $\left(\Proj{X}{}\otimes \mathcal{I}^Y\right)$ and $\left(\mathcal{I}^X \otimes \Proj{'Y}{}\right)$ are obviously also projectors with this property.
    
    Consider the \enquote{unravelled} version of Eq. \eqref{eq:PC}, Eq. \eqref{eq:PCunravelled}. We have seen that $\Dep{X_0}{}$ is such a projector, hence $\Dep{1-X_0}{}$ is also a projector of this kind by (a), so is $\Dep{X_1\left(1-X_0\right)}{}$ by (b), and so is $\Dep{1-X_1\left(1-X_0\right)}{}$ by (a) again. This proves the lemma in the case $n_X=1$ (that is, for Eq. \eqref{eq:app:P^1}). The general case follows by induction: if it is true for $\Proj{X}{n_X-1}$, then it is true for $\DepPar{X_{2n_X-2}}{\Proj{X}{n_X-1}}$ by (b), which is true for  $\mathcal{I}-\DepPar{X_{2n_X-2}}{ \Proj{X}{n_X-1} }$ by (a), which is again true for $ \DepPar{X_{2n_X-1}}{ \mathcal{I}-\DepPar{X_{2n_X-2}}{ \Proj{X}{n_X-1} } }$ by (b), and which is true for $\mathcal{I} - \DepPar{X_{2n_X-1}}{ \mathcal{I}-\DepPar{X_{2n_X-2}}{ \Proj{X}{n_X-1} } }$ by (a). This is Eq. \eqref{eq:PCunravelled} for $n_X$, hereby proving the induction.
\end{proof}
%
For example, in the case of a single party with one operation $O= \sum_{i_0i_1} o_{i_0 i_1} \; \GGB{X_0}{i_0} \otimes \GGB{X_1}{i_1}$, one has $\ProjOn{X}{1}{O} = \Dep{1-X_1+X_0X_1}{O} = o_{00} \; \GGB{X_0}{0}\otimes \GGB{X_1}{0} + \sum_{\mathbf{i}=(i_0,i_1>0)} o_{i_0i_1} \; \GGB{X_0}{i_0}\otimes \GGB{X_1}{i_1}$; the removed terms have indices $\mathbf{i} = (i_0>0,i_1=0)$. 

In the general case for a single party, we will write the action of a projector on the basis expansion as $\ProjOn{X}{n_X}{\sum_{\mathbf{i}} o_{\mathbf{i}}\;\sigma_{\mathbf{i}}^X} = \sum_{\mathbf{i} \in \{\{M^X\}\}} o_{\mathbf{i}}\; \sigma_{\mathbf{i}}^X$, where $\sum_{\mathbf{i} \in \{\{M^X\}\}}$ is to be understood as \enquote{summing only over the basis elements that belong to the subspace in which the set of $n_X$-combs $\{M^X\}$ is defined}. In the 1-node example of above, $\mathbf{i} \in \{\{M^X\}\}$ is thus equivalent to $\mathbf{i} \in \{(0,0)\} \cup \{(i_0,i_1)\}_{i_0=0,i_1>0}^{d^2_{X_0}-1,d^2_{X_1}-1}$. %Therefore, any valid comb has a decomposition restricted to a subset of the basis elements: $M = \sum_{\mathbf{i} \in \{M\}} m_{\mathbf{i}} \sigma_{\mathbf{i}}^X$.
%Notice that the $\mathbf{i}=\mathbf{0}$ coefficient always belongs to $\{\{M^X\}\}$. This can be seen in the structure of the projector \eqref{eq:PC}: there is always $2n_X + 1$ elements in the sum of subscripts, and each element acts in particular on $\mathbf{0}$. Hence, there is $n_X$ elements `removing' the $\mathbf{0}$ coefficient (\textit{i.e.} the negative terms in the sum) and $n_X+1$ `adding' it back (the positive terms). In the example, $\Dep{1}{}$ allows all coefficients so in particular $\mathbf{0}$, then $\Dep{-X_1}{}$ removes it together with all elements for which $\mathbf{i}=(i_0,i_1=0)$, and finally $\Dep{X_0X_1}{}$ add back $\mathbf{i}=(i_0=0,i_1=0)\equiv \mathbf{0}$ \footnote{Actually, the last element of Eq.\eqref{eq:PC} is always of the form \enquote{ $+\,\mathcal{D}$ }, so its action on the $\{\sigma_{\mathbf{i}}\}$ basis expansion is always to bring back the basis element $\sigma_{\mathbf{0}}$ (which amounts for the trace) after it was `added' and `removed' $n_X$ times by the other elements.}.

We next observe that the subspace spanned by the operators that are a tensor product of valid deterministic combs for the separate parties is the subspace on which the projector $\Proj{}{} \equiv \bigotimes_{X\in\mathfrak{N}} \Proj{X}{n_X}$ projects. Indeed, the action of $\mathcal{P}$ on an operator is to remove all terms in its Hilbert-Schmidt expansion that are not tensor products of terms allowed (left intact) by the local projectors $\Proj{X}{n_X}$. In other words, $\Proj{}{}$ projects on the subspace spanned by the tensor products of all locally allowed basis elements. Since each locally allowed basis element can be expressed as a linear combination of local deterministic combs, every operator in the subspace on which $\Proj{}{}$ projects is of the form $M= \sum_k q_k \left( \bigotimes_X M^X \right)_k$, where $M^X$ is a valid deterministic comb associated with party $X$, and $q_k$ are real coefficients. Conversely, every operator of this form is obviously left invariant by $\mathcal{P}$.
The trace of this last expression gives $\TrX{}{M} = \sum_k q_k \left( \prod_{X\in\mathfrak{N}} d_{X_{in}} \right)_k$, where for each $k$ the terms in parenthesis are exactly the input dimension of the Hilbert space, so they can be factored out of the sum: $\TrX{}{M} = d_{in} \sum_k q_k$. Hence, requiring that the trace is equal to $d_{in} \equiv \prod_{X\in\mathfrak{N}} d_{X_{in}}$ is equivalent to requiring that $\sum_k q_k=1$. Therefore, conditions \eqref{eq:AffineCombs} are equivalent to requiring that $M$ is an affine sum of tensor products of deterministic quantum combs. 

We will now prove the necessity of \eqref{eq:complProj} by using this observation to compute the quasiorthogonal projector explicitly. Let $M$ be an operator on $\LinOp{\Hilb{}}$ that satisfies conditions \eqref{eq:AffineCombs}. It is written as
\begin{equation}
    M= \bigotimes_{X\in \mathfrak{N}} \left( \sum_{\mathbf{i}_X \in \{\{M^X\}\}} m_{\mathbf{i}_X}\; \GGB{X}{\mathbf{i}_X} \right) \equiv \sum_{\mathbf{i}\in \{\{M\}\}} m_{\mathbf{i}}\; \GGB{}{\mathbf{i}} \,,
\end{equation}
where we have introduced a shortened formulation by making the tensor product implicit. Let there be an arbitrary operator $W = \sum_{\mathbf{j}} w_{\mathbf{j}} \sigma_{\mathbf{j}}$, where $\mathbf{j}$ is a multi-index defined analogously to $\mathbf{i}$. Applying the normalisation condition \eqref{eq:MPM_norm} on $W$ is equivalent to normalising it on all affine sums of tensor product of deterministic combs (see main text), hence Eq. \eqref{eq:MPM_norm_affine} gives
\begin{equation}\label{eq:Tr(WM)}
    \TrX{}{W\cdot M} = \sum_{\mathbf{j}} \sum_{\mathbf{i} \in \{\{M\}\}} w_{\mathbf{j}} m_{\mathbf{i}}\; d \;\delta_{{\mathbf{j}},\mathbf{i}} = 1\,.
\end{equation}
Since $\TrX{}{W} = w_{\mathbf{0}}d$ and $\TrX{}{M} = m_{\mathbf{0}}d$, the values of these two coefficients are fixed using Eqs. \eqref{eq:app:QuComb_normalisation} and \eqref{eq:app:W_norm} obtained above. This allows us to write
\begin{equation}
\begin{aligned}
    \sum_{\mathbf{j}} \sum_{\mathbf{i} \in \{\{M\}\}} w_{\mathbf{j}} m_{\mathbf{i}} d \delta_{\mathbf{j},\mathbf{i}} &= \sum_{\mathbf{i} \in \{\{M\}\}} w_{\mathbf{i}} m_{\mathbf{i}} d \\
    &= w_{\mathbf{0}}m_{\mathbf{0}} d +  \sum_{\mathbf{i} \neq \mathbf{0} \in \{\{M\}\}} w_{\mathbf{i}} m_{\mathbf{i}} d \\
    &= 1 + \sum_{\mathbf{i} \neq \mathbf{0} \in \{\{M\}\}} w_{\mathbf{i}} m_{\mathbf{i}} d\,,
\end{aligned}
\end{equation}
turning the normalisation condition into
\begin{equation}\label{eq:app:normWM}
    \sum_{\mathbf{i} \neq \mathbf{0} \in \{\{M\}\}} w_{\mathbf{i}} m_{\mathbf{i}} d = 0\,.
\end{equation} 
As $w_{\mathbf{i}}, m_{\mathbf{i}} \in \mathbb{R} \; \forall \mathbf{i}$ (since $W$ and $M$ are Hermitian), as $d$ is a non-negative integer, and as in general $m_{\mathbf{i}} \neq 0$ for at least one given value of $\mathbf{i} \neq \mathbf{0}$ (otherwise we are back to the case $M= \frac{\mathds{1}}{\prod d_{X_{out}}}$), we are left with two possibilities: either $\sum_{\mathbf{i} \neq \mathbf{0} \in \{\{M\}\}} w_{\mathbf{i}} m_{\mathbf{i}}=0$ for some nonvanishing $w_{\mathbf{i}}$, or $ w_{\mathbf{i}} = 0 \,, \forall \mathbf{i} \neq \mathbf{0} \in \{\{M\}\}$. We will show that only the second possibility is viable.

Following Ref. \cite{OG2016}, one can always construct a valid deterministic quantum comb of the form $M_{\mathbf{a}} = m_{\mathbf{0}} \GGB{}{{\mathbf{0}}} + m_{\mathbf{a}} \GGB{}{\mathbf{a}}$ for $\mathbf{a} \neq {\mathbf{0}} \in \{\{M\}\} $ with a small enough $ m_{\mathbf{a}}$ coefficient so that Eqs. \eqref{eq:QuComb} are satisfied (it is sufficient to set $m_{\mathbf{0}}$ to $\left(\prod d_{X_{out}}\right)^{-1}$ and $m_{\mathbf{a}}^2 \leq m_{\mathbf{0}}^2$). Then, equation \eqref{eq:app:normWM} yields $w_{\mathbf{a}} = 0$. Doing it again with a different valid comb $M_{\mathbf{b}} = m_{\mathbf{0}} \GGB{}{{\mathbf{0}}} + m_{\mathbf{b}} \GGB{}{\mathbf{b}}$ such that $\mathbf{b} \neq \mathbf{a}$ yields a second condition, $w_{\mathbf{b}} = 0$. Repeating this argument for all possible choice of basis element, $\left\{ M_{\mathbf{k}} = m_{\mathbf{0}} \GGB{}{{\mathbf{0}}} + m_{\mathbf{k}} \GGB{}{\mathbf{k}} \right\}_{\mathbf{k}\neq{\mathbf{0}} \in \{\{M\}\}}$, proves the latter possibility: $w_{\mathbf{i}} = 0 \,, \forall \; {\mathbf{i}} \neq {\mathbf{0}} \; \in \{\{M\}\}$. 

Note that the last condition defines a subspace in the space of operators to which $W$ must belong. This subspace is quasiorthogonal to the subspace $\mathrm{Span}\left\{ \bigotimes M\right\}$, meaning that the intersection of the two subspaces is the span of the unit matrix. Noticing that $w_{\mathbf{0}} \sigma_{\mathbf{0}} = \Dep{X}{W}\equiv \mathcal{D}[W]$, one expresses this last statement in a basis-independent formulation:
\begin{multline}\label{eq:W}
   \{W\}: \sum_{\mathbf{i} \in \{\{M\}\}} w_{\mathbf{i}} \GGB{}{\mathbf{i}} = w_{\mathbf{0}} \GGB{}{{\mathbf{0}}} \\
   \iff \left( \Proj{}{} - \mathcal{D}\right)[W]= 0 \,.
\end{multline}
One can check that $\left( \Proj{}{} - \mathcal{D}\right)^2 = \Proj{}{} - \mathcal{D}$, so $\Proj{}{} - \mathcal{D}$ is a projector. Taking the orthogonal complement, one gets
\begin{equation}
    W = \left(\mathcal{I} - \mathcal{P} + \mathcal{D} \right) [W] \,, \label{eq:oui}
\end{equation}
which is the sought formula.

The fact that Eqs. \eqref{eq:complProj} and \eqref{eq:norm} are sufficient for \eqref{eq:MPM_norm_affine} (and therefore \eqref{eq:MPM_norm}) is straightforward to check. Indeed, plugging \eqref{eq:W}, which is equivalent to \eqref{eq:complProj}, together with \eqref{eq:norm} in Eq. \eqref{eq:Tr(WM)}, one verifies that $m_{\mathbf{0}} \frac{d}{d_{in}} = 1$ because Eq. \eqref{eq:AffineCombs_norm} implies that $m_{\mathbf{0}} = 1/d_{out}$. This completes the proof of the theorem.

==> Version 2.0 sent to Quantum/APP2.tex <==
\section{Proof of Theorem \ref{theo:PV=UPTildeC} \label{app:proof:V=UC}}
The proof will be split among several lemmas. Given a finite set of orthogonal projectors $\Proj{1}{},\Proj{2}{},\ldots$, we call their \textit{intersection} the orthogonal projector $\Proj{}{\Proj{1}{}\cap\Proj{2}{} \cap \ldots}$ that projects on the intersection of the subspaces on which $\Proj{1}{},\Proj{2}{},\ldots$ project. As shown in \cite{Piziak1999}, if the projectors commute, this intersection is given by the \enquote{product} of the projectors (formally, their composition): 
\begin{equation}
    \Proj{}{\Proj{1}{}\cap\Proj{2}{} \cap \ldots} \equiv \Proj{1}{}\cap\Proj{2}{} \cap \ldots = \Proj{1}{}\Proj{2}{}\ldots \quad .
\end{equation}
Let $\Proj{A\prec B}{n_A+n_B}$ be the projector on the space of valid $(n_A+n_B)$-combs formed by composing $n_A$ operations (or \enquote{teeth}) of a party $A$ with the $n_B$ operations of another party $B$ into an overall deterministic $(n_A+n_B)$-comb where the operations of Alice are all before those of Bob (see the second case from the left in Fig. \ref{fig:CombCompo} for a graphical example). Let $\Proj{B \prec A}{n_A+n_B}$ be the same kind of comb projector but where the operations of $B$ are put before those of $A$ (rightmost case in Fig. \ref{fig:CombCompo}). Then the intersection of these two projectors is
\begin{equation}\label{eq:proj_inter}
    \Proj{A\prec B}{n_A+n_B} \cap \Proj{B \prec A}{n_A+n_B} = \Proj{A\prec B}{n_A+n_B}\Proj{B \prec A}{n_A+n_B} \, .
\end{equation}

%We will simplify the notation when the teeth are ordered party-wise, \textit{e.g.} writing $A\prec B$ instead of $\Party{A}{1}{} \prec \Party{B}{1}{} \prec \Party{B}{2}{}$ like in Fig. \ref{fig:CombCompo}.
%
\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{A1.png}
    \caption{Examples of ways to append $n_A=1$ operations of Alice with $n_B=2$ operations of Bob into valid 3-combs, with the associated projectors on a particular subspace of valid 3-comb written below its graphical representation.}
    \label{fig:CombCompo}
\end{figure}
%

Any comb in the intersection should therefore be compatible with either all the operations of Alice being first or those of Bob. Intuitively, one can conceive that the only kind of combs valid within this requirement are those where the part of Alice is forbidden to communicate with the part of Bob and vice versa. This is the content of the first lemma.
\begin{lemm} \label{lem:tensorcombs}
    Consider a quantum comb in which some of the teeth are associated with a party $A$ and the others with $B$. Then, the intersection of the subspace of deterministic quantum combs in which the teeth of $A$ are all before those of $B$ (\textit{e.g.} Fig. \ref{fig:CombCompo}, second case from the left) with the one in which the teeth of $B$ are all before those of $A$ (Fig. \ref{fig:CombCompo}, rightmost case) is equivalent to $\mathrm{Span}\left\{ M^A \otimes M^B \right\}$, which is the subspace spanned by the tensor product of a smaller deterministic comb acting on the nodes of $A$ only together with a smaller deterministic comb acting on the nodes of $B$ only (Fig. \ref{fig:CombCompo}, leftmost case). This is because their projectors are equivalent:
    \begin{equation}
        \Proj{A\prec B}{n_A+n_B}\Proj{B \prec A}{n_A+n_B} = \Proj{A}{n_A} \otimes \Proj{B}{n_B} \,.%
        \label{eq:lem:V=UC.1}%
    \end{equation}
\end{lemm}
\begin{proof}
    The proof relies upon the recursive formulation of a quantum comb projector \eqref{eq:PC}. When inspecting formula \eqref{eq:PCunravelled} for $\Proj{A\prec B}{n_A+n_B}$, we see that it is possible to express the projector as: 
    \begin{equation}\label{eq:app:projAB}
        \Proj{A\prec B}{n_A+n_B} = \mathcal{I}^A \otimes \Proj{B}{n_B} - \left(\mathcal{I}^A - \Proj{A}{n_A}\right) \otimes \mathcal{D}^B \,.
    \end{equation}
    Indeed, it holds for the case $n_B=1$:
    \begin{equation}
    \begin{aligned}
        \Proj{A\prec B}{n_A+1} &= \DepPar{1-B_{1}}{\cdot} + \DepPar{B_0B_1}{\Proj{A}{n_A}}\\
        &=\DepPar{1-B_{1}+B_0B_1}{\cdot} - \DepPar{B_0B_1}{1-\Proj{A}{n_A}}\\
        &=\mathcal{I}^A \otimes \Proj{B}{1} - \DepPar{B_0B_1}{\mathcal{I}^A - \Proj{A}{n_A}}\\
        &=\mathcal{I}^A \otimes \Proj{B}{1} - \left(\mathcal{I}^A - \Proj{A}{n_A}\right) \otimes \mathcal{D}^B \,.
    \end{aligned}
    \end{equation}
    Suppose the decomposition \eqref{eq:app:projAB} is true for $n_A+n_B-1$ operations. We define the projector for such a case as $\Proj{A\prec B}{n_A+n_B-1} \equiv \Proj{A\prec \Party{B}{1}{} \prec \ldots \prec \Party{B}{n_B-1}{}}{n_A+n_B-1}$. Then, for $n_A+n_B$:
    \begin{multline}
        \Proj{A\prec B}{n_A+n_B} = \DepPar{1-B_{2n_B-1}}{\cdot} + \DepPar{B_{2n_B-2}B_{2n_B-1}}{\Proj{A\prec B}{n_A+n_B-1}}\\
        = \DepPar{1-B_{2n_B-1}}{\cdot} + \DepPar{B_{2n_B-2}B_{2n_B-1}}{\mathcal{I}^A \otimes \Proj{B}{n_B-1}}\\
        - \DepPar{B_{2n_B-2}B_{2n_B-1}}{\left(\mathcal{I}^A - \Proj{A}{n_A}\right) \otimes \mathcal{D}^B_{n_B-1}}\\
        = \mathcal{I}^A \otimes \Proj{B}{n_B} - \left(\mathcal{I}^A - \Proj{A}{n_A}\right) \otimes \mathcal{D}^B_{n_B}\,,
    \end{multline}
    where we injected $\Proj{A\prec B}{n_A+n_B-1} = \mathcal{I}^A \otimes \Proj{B}{n_B-1} - \left(\mathcal{I}^A - \Proj{A}{n_A}\right) \otimes \mathcal{D}^B_{n_B-1}$ to go from the first equality to the second, with $\mathcal{D}^B_{n_B-1} \equiv \Dep{B_0\ldots B_{2n_B-3}}{}$. Next, we used Eq. \eqref{eq:PC} together with $\DepPar{B_{2n_B-2}B_{2n_B-1}}{\mathcal{D}^B_{n_B-1}} = \mathcal{D}^B$ to go to the last equality. This proves decomposition \eqref{eq:app:projAB} by induction.
    
    Now, applying an analogous decomposition to $\Proj{B\prec A}{n_A+n_B}$, the left-hand side of Eq. \eqref{eq:lem:V=UC.1} becomes
    \begin{multline}
        \Proj{A \prec B}{n_A+n_B}\Proj{B \prec A}{n_A+n_B} =\\
        \left( \mathcal{I}^A \otimes \Proj{B}{n_B} - \left(\mathcal{I}^A - \Proj{A}{n_A}\right) \otimes \mathcal{D}^B \right)\\
        \times \left( \Proj{A}{n_A} \otimes \mathcal{I}^B - \mathcal{D}^A \otimes \left(\mathcal{I}^B - \Proj{B}{n_B}\right) \right)\\
        = \Proj{A}{n_A} \otimes \Proj{B}{n_B}\,. 
    \end{multline}
    To go to the last line, we used the fact that $\mathcal{D}$ is the absorbing (\textit{i.e.} \enquote{zero}) element of the multiplication in the ring (see Sec. \ref{app:projo}), making all the terms where it appears vanish, since $\left(\mathcal{I}^X - \Proj{X}{}\right)\mathcal{D}^X = \left( \mathcal{D}^X - \mathcal{D}^X\right) = 0$. 
\end{proof}
%
%We also use the notation $A \nprec B$ to indicate that a party $A$ is explicitly in the causal future of $B$, which implies that $A$ cannot signal to $B$. This is to write $\Proj{A}{n_A} \otimes \Proj{B}{n_B} \equiv \Proj{A \nprec \nsucceq B}{n_A+n_B}$ to emphasise the fact that subsystems $A$ and $B$ in the overall $n_A+n_B$-comb cannot signal to each other within the comb. 
The projector of this first lemma is simply the projector on a subspace containing all the $(n_A+n_B)-$combs obtained by taking the tensor product of an $n_A$-comb with an $n_B$-comb (\textit{e.g.} leftmost case in Fig. \ref{fig:CombCompo}). It should also be compatible with permutations of Bob's and Alice's teeth in the full comb that respect the local causal ordering for each party. We will need the $\pi_i(A,B)$ notation introduced in Sec. \ref{sec:MPM=Combs} to refer to the $i$-th valid permutation in the causal ordering of the teeth of parties $A$ and $B$ in order to express this as a corollary.
%
\begin{coro}\label{coro:V=UC.1}
The subspace made by the intersection of the $(n_A+n_B)$-combs such that all the teeth of $A$ are before those of $B$ with the $(n_A+n_B)$-combs such that all the teeth of $B$ are before those of $A$ is inside the subspace of all $(n_A+n_B)$-combs whose teeth orderings are permutations of the teeth of $A$ and $B$ that respect the local order assumed for $A$ and $B$:   
    \begin{equation}\label{eq:coro:V=UC.1}
        \Proj{A\prec B}{n_A+n_B}\Proj{B \prec A}{n_A+n_B}\Proj{\pi_i(A, B)}{n_A+n_B} = \Proj{A\prec B}{n_A+n_B}\Proj{B \prec A}{n_A+n_B}\, \forall i \,.
    \end{equation}
\end{coro}
\begin{proof}
    The subset of deterministic quantum combs on $\LinOp{\Hilb{A} \otimes \Hilb{B}}$ formed by the tensor product of combs on $A$ and $B$ is automatically a valid comb, no matter how one defines the relative ordering between the teeth of $A$ and $B$ \cite{Chiribella2009}. %In set notation one can sketch the proof as $\forall \pi_i: \, (A\prec B \cap B \prec A) \subset \pi_i(A\prec B) \Rightarrow A\prec B \cap B \prec A \cap \pi_i(A\prec B) = A\prec B \cap B \prec A$. %for all $i$. 
\end{proof}
%
In other words, this corollary says that when an operator is a tensor product of a deterministic $n_A$-comb with a deterministic $n_B$-comb, then it is a valid deterministic $(n_A+n_B)$-comb for any ordering of the teeth compatible with the partial ordering of the individual combs.


The second lemma needed is just a simplification of the formula for the union of projectors when applied to the case of quasiorthogonal projectors for different teeth orderings. 
\begin{lemm}\label{lemm:UPtilde=1-P+D}
    The union of two arbitrary quasiorthogonal projectors $\CompProj{\pi_i(A,B)}{n_A+n_B}$ and $\CompProj{\pi_j(A,B)}{n_A+n_B}$ is given by%
    \begin{equation}\label{eq:lem:V=UC.2}
        \CompProj{\pi_i(A, B)}{n_A+n_B} \cup \CompProj{\pi_j(A, B)}{n_A+n_B} = \mathcal{I} - \Proj{\pi_i(A, B)}{n_A+n_B} \Proj{\pi_j(A, B)}{n_A+n_B} + \mathcal{D} \,.
    \end{equation}%
\end{lemm}
\begin{proof}
    It is proven by doing the computation explicitly, then simplifying by using again the fact that the projector $\mathcal{D}$ on the span of unity is the zero element. Hence,
	\begin{equation}    
    \begin{aligned}
        \CompProj{\pi_i}{} \CompProj{\pi_j}{} &= \left(\mathcal{I} - \Proj{\pi_i}{} + \mathcal{D}\right) \left(\mathcal{I} - \Proj{\pi_j}{} + \mathcal{D}\right)\\
        &= \mathcal{I} - \Proj{\pi_i}{} - \Proj{\pi_j}{} + \Proj{\pi_i}{}\Proj{\pi_j}{} + \mathcal{D}\,,
    \end{aligned}    
    \end{equation}
    where we have dropped the $n_A+n_B$ subscript and simplified the superscript (\textit{i.e.} $\pi_i(A, B) \equiv \pi_i$ ) in order to shorten the notation. This gives, when plugged into \eqref{eq:UprojCtilde},
    \begin{equation}
    \begin{aligned}
        \CompProj{\pi_i}{} \cup \CompProj{\pi_j}{} &= \mathcal{I} - \Proj{\pi_i}{} + \mathcal{D} + \mathcal{I} - \Proj{\pi_j}{} + \mathcal{D} \\
        & \quad - \left(\mathcal{I} - \Proj{\pi_i}{}  - \Proj{\pi_j}{} + \Proj{\pi_i}{}\Proj{\pi_j}{} + \mathcal{D} \right)\\
        &= \mathcal{I} - \Proj{\pi_i}{} \Proj{\pi_j}{} + \mathcal{D}\,.
    \end{aligned}    
    \end{equation}
\end{proof}

All the elements needed for the main proof are in place. Note that the lemmas have been derived assuming only 2 parties. Actually, these hold analogously for any number of parties, since every formula that was used is associative. In the case where $|\mathfrak{N}|>2$, one just has to group the parties together to get back to the 2-partite scenario.

For the main proof, we start from the right-hand side of equation \eqref{eq:PV=UPTildeC} to which we apply the result of Lemma \ref{lemm:UPtilde=1-P+D}, equation \eqref{eq:lem:V=UC.2}:
\begin{equation}
    \bigcup_{\pi_i} \CompProj{\pi_i(A,B, \ldots)}{n_A+n_B+ \ldots} = \mathcal{I} - \prod_{\pi_i} \Proj{\pi_i(A,B,\ldots)}{n_A+n_B+ \ldots} +\mathcal{D} \, .
\end{equation}
We then apply Corollary \ref{coro:V=UC.1} so the permutations $\pi_i$ of all the nodes are restricted to permutations $\pi_i'$ of whole parties only:
%, which we note using $\pi_i'$, thus $\{\pi_i'\} \subset \{\pi_i\}$ where the permutations of single node like $\Party{A}{1}{} \prec \Party{B}{1}{} \prec \Party{A}{2}{}\prec \ldots$ are forbidden. 
	\begin{equation}
	\begin{aligned}
    \mathcal{I} - \prod_{\pi_i'} \Proj{\pi_i'(A,B, \ldots)}{n_A+n_B+ \ldots} &+\mathcal{D} =\\
    \mathcal{I} - &\Proj{A\prec B\prec \ldots}{n_A+n_B+ \ldots}\Proj{B \prec A\prec \ldots}{n_A+n_B+ \ldots}... +\mathcal{D} \,.
	\end{aligned}    
    \end{equation}
Remember that here a superscript $X$ is referring to $n_X$ nodes like $X \equiv \Party{X}{1}{}\prec\Party{X}{2}{}\prec \ldots \prec \Party{X}{n_X}{}$.
The final step is to apply Lemma \ref{lem:tensorcombs}, equation \eqref{eq:lem:V=UC.1}, yielding
\begin{multline}
    \mathcal{I} - \Proj{A\prec B\prec \ldots}{n_A+n_B+ \ldots}\Proj{B \prec A\prec \ldots}{n_A+n_B+ \ldots}\ldots +\mathcal{D} =\\
    \mathcal{I} - \left(\Proj{A}{n_A}\otimes \Proj{B}{n_B}\otimes \ldots\right) +\mathcal{D} \,.   
\end{multline}
We can now invoke the definition of the quasiorthogonal projector \eqref{eq:complProj} on the right-hand side, and we have proven that 
\begin{equation}
    \bigcup_{\pi_i} \CompProj{\pi_i(A,B, \ldots)}{n_A+n_B+ \ldots} = \prescript{Q}{}{\left(\Proj{A}{n_A}\otimes\Proj{B}{n_B}\otimes\ldots\right)}\quad .
\end{equation}
%
%\textit{Remark 4.} As we have noted in Remark 3, Section \ref{sec:charactMPM}, some of these results have been independently found in references \cite{Perinotti2016,Bisio2018}. Noticeably, the content of Lemma \ref{lem:tensorcombs} is similar to Lemma 5 of \cite{Bisio2018}, while the one of Corollary \ref{coro:V=UC.1}

==> Version 2.0 sent to Quantum/APP3.tex <==
\section{Details for the MPM definition of causal separability\label{app:CnS}}
%
For completeness, we show explicitly that the correlations obtained through the `Born rule' \eqref{eq:MPMBorn} for MPMs can be transformed into correlations obtained with a PM extended by identity side channels. We will make use of a version of the \textit{link product} \cite{Chiribella2009}, which allows to merge combs together. In the context of our basis-independent convention for the CJ isomorphism, we define the link product between two operators $M^{CB}$ and $N^{B^*A}$, where $A$ and $C$ are separate systems or the trivial system, and $B$ and $B^*$ are mutually dual (\textit{i.e.} $\mathcal{H}^{B^*}$ and $\mathcal{H}^{B}$ are Hilbert spaces dual to each other, assuming the canonical isomorphism $(\mathcal{H}^*)^* \cong \mathcal{H}$ in the finite-dimensional case), as%
\begin{equation}\label{linkproduct}%
    \begin{gathered}%
         L^{AC} = M^{CB} \ast N^{B^* A}    : = \\
        \TrX{B B^*}{\left(M^{CB} \otimes N^{B^* A}\right) \left(\mathds{1}^{CB} \otimes Id^{BB^*}\right)},
    \end{gathered}%
\end{equation}
where $Id^{BB^*} \equiv \sum_{ij}^{d_B}  \dyad{ii}{jj}^{BB^*}$. 

Consider a quantum 2-comb $M^A\equiv M^{A_0A_1A_2A_3}$. The CP map it describes can be seen as resulting from the composition of two CP maps with an intermediate identity side channel. In the CJ representation, this is given by the link product between the corresponding 1-combs,
\begin{equation}
    M^A = M^{A_3A_2L_2} \ast Id^{L_2^*L_1^*} \ast M^{L_1A_1A_0} \quad , \label{eq:app:M^A}
\end{equation}
where $L_1^*$ is the ancillary output system of the first CP map (with CJ operator $M^{L_1A_1A_0}$), $L_2$ is the ancillary input system of the second CP map (with CJ operator $M^{A_3A_2L_2}$), and $Id^{L_2^*L_1^*}$ is the CJ operator of the identity side channel connecting these systems. 

This is explicitly given by
\begin{widetext}
\begin{equation*}
    M^A = \TrX{L_2L_2^*L_1L_1^*}{\left(M^{A_3A_2L_2} \otimes Id^{L_2^*L_1^*} \otimes  M^{L_1 A_1A_0}\right) \left(\mathds{1}^{A_3A_2} \otimes  Id^{L_2L_2^*} \otimes Id^{L_1^*L_1} \otimes \mathds{1}^{A_1A_0}\right)}.
\end{equation*}
\end{widetext}
Computing the trace over $L_2^*L_1^*$ yields
\begin{equation}\label{eq:app:LinkalaOO}
    M^A = \TrX{L_2 L_1}{\left(M^{A_3A_2L_2} \otimes M^{L_1 A_1A_0}\right) \left(\mathds{1}^{A} \otimes Id^{L_2L_1}\right)}.
\end{equation}
In this last expression, $Id^{L_2L_1} \equiv \sum_{ij}^{d_L^2} \dyad{ii}{jj}^{L_2L_1}$ is the \textit{transpose} of the CJ operator of an identity channel from $\Hilb{L_1^*}$ to $\Hilb{L_2}$ (just like a PM is the transpose of the CJ operator of a channel from the outputs of nodes to the inputs of nodes).  

Plugging equation \eqref{eq:app:LinkalaOO} into the `Born rule' between the 2-comb $M^A$ and a 2-node MPM $W$, one has 
\begin{equation}\label{eq:app:split}
    \TrX{}{M^A W} = \TrX{}{\left( M^{A_3A_2L_2} \otimes M^{L_1A_1A_0} \right) \left( W \otimes Id^{L_2L_1} \right)} ,
\end{equation}
where $ M^{A_3A_2L_2}, M^{L_1A_1A_0} $ are quantum 1-combs, and $ W \otimes Id^{L_2L_1} $ can be shown to be a valid (M)PM, hinting the formula \eqref{eq:MPMintoPM} for the general case. Indeed, formula \eqref{eq:app:M^A} can be applied repetitively in the case of a party with more than 2 nodes: $M^A = M^{{A}_{2n_A-2}{A}_{2n_A-1}{L}_{2n_A-2}} \ast\ldots    \ast M^{L_3A_3A_2L_2} \ast Id^{L_2^*L_1^*}\ast M^{{L}_{1}{A}_{1}{A}_{0}}$, and then the identity $\TrX{Y}{A^Y \cdot \TrX{X}{B^{XY}}} = \TrX{XY}{\left(\mathds{1}^X\otimes A^Y \right) B^{XY}}$ can be used to rewrite the whole expression as one overall partial trace. The tensor product being a special case of link product over the trivial system \cite{Chiribella2009}, this argument also applies to the multipartite case.

Consequently, the correlations achievable with an MPM are equivalent to those in a PM extended by side channels and we can appeal to the concept of causal separability for PMs in order to define causal separability for MPMs as it is done in Definition \ref{def:MPM_CnS}.

As shown in Ref. \cite{OG2016}, for the PM definition of causal separability, the possibility of extending the local operations of the parties to act on local ancillary input systems that may be entangled with the ancillary input systems of other parties also needs to be considered. Neglecting to do so may mistakenly lead to the conclusion that a PM is causally separable, although it is able to violate a causal inequality when using such an extension. Likewise, we have shown in the main text that neglecting the side channels lead to the same kind of problem. We end this appendix by reformulating Definition \ref{def:MPM_CnS} into one closer to Ref. \cite{OG2016,Wechs2018}, so that the consequences of local causal ordering are made explicit and extension by arbitrary ancillas and side channels is explicit.

We only need to rewrite \eqref{eq:app:split} as
\begin{equation}
    \TrX{}{M^A W} = \TrX{A_3A_2L_2}{M^{A_3A_2L_2} W_{|M^{L_1A_1A_0}}}\,,
\end{equation}
where we have defined the \textit{conditional process matrix} 
%
%
\begin{widetext}
\begin{equation}
    W_{|M^{L_1A_1A_0}} = c \;\TrX{L_1A_1A_0}{\left(  \mathds{1}^{A_3A_2L_2} \otimes M^{L_1A_1A_0} \right) (W\otimes Id^{L_2L_1})} \,.
\end{equation}
This can be shown to be a valid process matrix on the remaining node between $A_2L_2$ and $A_3$ for all the possible choices of $M^{L_1A_1A_0}$, as long as the normalisation factor is chosen such that Eq. \eqref{eq:norm} is verified. On the contrary, the analogously defined $W_{|M^{A_3A_2L_2}}$ will not always be a valid PM for all $M^{A_3A_2L_2}$ as it can lead to post-selection. This implies that when we reformulate the `Born rule' so as to make the unravelling from an $n$-node MPM to an $(n-1)$-node MPM apparent, starting the unravelling with a node that is not the first of some party is automatically forbidden. The generalisation of this unravelling procedure yields the following definition:
%
\begin{defi}[Causal separability of the MPM]\label{def:MPM_CS}
    Consider an MPM $W$ shared by $|\mathfrak{N}|$ parties. For $|\mathfrak{N}|=1$ this MPM is a deterministic quantum comb and thus causally separable. For $|\mathfrak{N}|>1$, the MPM is causally separable if and only if, for any state $\rho \in \LinOp{\bigotimes_{X\in\mathfrak{N}}\bigotimes_{i=0}^{n_X-1} \Hilb{X_{2i}'}}$ defined on an extension of the parties' input subsystems $\Hilb{X_{2i}} \rightarrow \Hilb{\tilde{X}_{2i}} = \Hilb{X_{2i}} \otimes \Hilb{X_{2i}'}$, the extended MPM can be decomposed as
    \begin{equation}
        W \otimes \rho = \sum_{X\in\mathfrak{N}} q_{\Party{X}{1}{}} W^{\rho}_{\Party{X}{1}{}}\,,
    \end{equation}
    with $q_{\Party{X}{1}{}}\geq0$, $\sum_{X\in\mathfrak{N}} q_{\Party{X}{1}{}} = 1$, and where $W^{\rho}_{\Party{X}{1}{}}$ is an MPM compatible with party $X$'s first operation being first in the causal unravelling (\textit{i.e.} there can be no signalling from the rest of the nodes to $\Party{X}{1}{}$ \cite{OG2016}), so that the conditional MPM after the first operation of $X$ has been carried out,
    \begin{equation}
        \left( W^{\rho}_{\Party{X}{1}{}}\right)_{\left|M^{X_0X'_0X_1L_1}\right.} = c \; \TrX{X_0X'_0X_1L_1}{\left( M^{X_0X'_0X_1L_1} \otimes \mathds{1} \right)\left( W^X \otimes \rho^{X'} \otimes Id^{L_2L_1} \right)} \,,
    \end{equation}
    is itself causally separable for all possible CP maps between $\LinOp{\Hilb{X_0}\otimes \Hilb{X'_0}}$ and $\LinOp{\left(\Hilb{X_1}\right)^* \otimes \left(\Hilb{L_1}\right)^*}$ represented by the CJ operator $M^{X_0X'_0X_1L_1}$. Here $L_2$ is an extension of the input system of $\Party{X}{2}{}$ and $c$ is a normalisation constant. %Subsystem $L_1$ (respectively, $L_2$) is the extension of the output system of $\Party{X}{1}{}$ (the input system of $\Party{X}{2}{}$) over which the side channel is defined.
\end{defi}
\end{widetext}

==> Version 2.0 sent to Quantum/APP4.tex <==
\section{Details for the activation example\label{app:exemple}}
As an illustration of Theorem \ref{theo:complement}, we will now sketch the proof that the operator \eqref{eq:Activable}, rewritten here for convenience
\begin{multline}
    W^{AB}=\\
    \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}}\left[\GGB{A_0}{x}\GGB{A_2}{z}\GGB{A_3}{z}\GGB{B_0}{z} + \GGB{A_0}{z}\GGB{A_2}{z}\GGB{B_1}{z}\right]\right)\,,
\end{multline}
is a valid MPM with 3 nodes, where $\Party{A}{1}{}\prec \Party{A}{2}{}$.

This is a PSD matrix with trace $\TrX{}{W^{AB}} = 8 = d_{A_1}d_{A_3}d_{B_1} = d_{out}$, so conditions \eqref{eq:pos} and \eqref{eq:norm} are directly verified. The projective condition \eqref{eq:complProj} is given by 
\begin{align}
    &W^{AB}=\mathcal{I}^{AB} \left[ W^{AB} \right]- \notag\\
    &\DepPar{\left(1-A_3+A_2A_3-A_1A_2A_3+A_0A_1A_2A_3\right)\left(1-B_1+B_0B_1\right)}{W^{AB}} \notag\\ 
    &+ \mathcal{D}^{AB} \left[ W^{AB} \right] \,, \label{eq:WAB}
\end{align}
where \eqref{eq:ProjComb} have been used to find the 2-comb projector on $A$, $\Proj{\Party{A}{1}{}\prec \Party{A}{2}{}}{2}= \Dep{\left(1-A_3+A_2A_3-A_1A_2A_3+A_0A_1A_2A_3\right)}{}$, as well as the 1-comb projector on $B$, $\Proj{B}{1}=\Dep{\left(1-B_1+B_0B_1\right)}{}$.
Notice that $\DepPar{A_3}{W^{AB}} = \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}} \GGB{A_0}{z}\GGB{A_2}{z}\GGB{B_1}{z}\right)$, and $\DepPar{B_1}{W^{AB}} = \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}}\GGB{A_0}{x}\GGB{A_2}{z}\GGB{A_3}{z}\GGB{B_0}{z} \right)$, while all the other combinations of prescripts are equivalent to the action of $\mathcal{D}^{AB}$ on the matrix, \textit{i.e.} $\DepPar{A_3B_1}{W^{AB}} = \DepPar{B_0B_1}{W^{AB}} = \DepPar{A_2A_3}{W^{AB}}=\ldots = \frac{\mathds{1}}{8} = \mathcal{D}^{AB} \left[ W^{AB} \right]$. This allows us to simplify the projective condition \eqref{eq:WAB} into
\begin{equation}
    W^{AB} = W^{AB} - \DepPar{1-A_3-B_1}{W^{AB}} - \mathcal{D}^{AB} \left[ W^{AB} \right]\,,
\end{equation}
which is effectively verified:
\begin{multline}
    W^{AB} =\DepPar{A_3}{W^{AB}} + \DepPar{B_1}{W^{AB}} - \mathcal{D}^{AB} \left[ W^{AB} \right]\\
    =\frac{\mathds{1}}{4}+\frac{1}{8\sqrt{2}}\left[\GGB{A_0}{x}\GGB{A_2}{z}\GGB{A_3}{z}\GGB{B_0}{z} + \GGB{A_0}{z}\GGB{A_2}{z}\GGB{B_1}{z}\right] - \frac{\mathds{1}}{8}\\
    =\frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}}\left[\GGB{A_0}{x}\GGB{A_2}{z}\GGB{A_3}{z}\GGB{B_0}{z} + \GGB{A_0}{z}\GGB{A_2}{z}\GGB{B_1}{z}\right]\right).
\end{multline}

The same way, operator \eqref{eq:Activated}, 
\begin{multline}
    W= \\
    \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}}\left[\GGB{A_2}{z}\GGB{A_3}{z}\GGB{L_2}{x}\GGB{B_0}{z} + \GGB{A_2}{z}\GGB{L_2}{z}\GGB{B_1}{z}\right]\right) \,,
\end{multline}
written here without superscript, will now be proven to be a valid (M)PM on 2 nodes $A$ and $B$, where $L_2$ is extending the input system of party $A$. It is straightforward to check that it is a PSD matrix with $\TrX{}{W} = 4 = d_{A_3}d_{B_1}$, hence verifying \eqref{eq:pos} and \eqref{eq:norm}. The projective condition \eqref{eq:complProj} is expressed as
\begin{multline}
     W =\\
      \mathcal{I} \left[ W \right]-\DepPar{\left(1-A_3+L_2A_2A_3\right)\left(1-B_1+B_0B_1\right)}{W} +\mathcal{D} \left[ W\right] = \\
     \DepPar{A_3+B_1-A_3B_1+A_3B_0B_1-B_0B_1+L_2A_2A_3B_1-L_2A_2A_3}{W}\,. \label{eq:non}
\end{multline}
Computing each term on the right hand side, we find
\begin{equation}
\begin{aligned}
    &\Dep{A_3}{W} = \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}} \GGB{A_2}{z}\GGB{L_2}{z}\GGB{B_1}{z}\right) ,\\
    &\Dep{B_1}{W} = \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}}\GGB{A_2}{z}\GGB{A_3}{z}\GGB{L_2}{x}\GGB{B_0}{z} \right) ,\\
    &\Dep{A_3B_1}{W} = \Dep{A_3B_0B_1}{W}  = \Dep{L_2A_2A_3B_1}{W} = \Dep{L_2A_2A_3}{W} =\\
    &\quad\Dep{B_0B_1}{W} = \frac{\mathds{1}}{8}\,.
\end{aligned}
\end{equation}
Therefore, \eqref{eq:non} becomes
\begin{multline}
    W = \Dep{A_3}{W}+\Dep{B_1}{W}-\Dep{A_3B_1}{W}\\
    = \frac{\mathds{1}}{4}+\frac{1}{8\sqrt{2}} \left[\GGB{A_2}{z}\GGB{L_2}{z}\GGB{B_1}{z}+\GGB{A_2}{z}\GGB{A_3}{z}\GGB{L_2}{x}\GGB{B_0}{z}\right]- \frac{\mathds{1}}{8}\\
    = \frac{1}{8}\left(\mathds{1}+\frac{1}{\sqrt{2}}\left[\GGB{A_2}{z}\GGB{A_3}{z}\GGB{L_2}{x}\GGB{B_0}{z} + \GGB{A_2}{z}\GGB{L_2}{z}\GGB{B_1}{z}\right]\right) \,, 
\end{multline}
proving that the projective condition \eqref{eq:complProj} is indeed verified for $W$.

==> Version 2.0 sent to Quantum/commands.tex <==
\newcommand{\Herm}[1]{\text{Herm}\left( #1 \right)}
\newcommand{\Hilb}[1]{\mathcal{H}^{#1}}
\newcommand{\LinOp}[1]{\mathcal{L}\left( #1 \right)}
\newcommand{\LinOpA}[2]{\mathcal{L}\left( \left( #1 \right) \rightarrow \left( #2 \right) \right)}
\newcommand{\LinOpB}[2]{\mathcal{L}\left( #1 \rightarrow  #2 \right)}
\newcommand{\MapX}[2]{ \frac{\mathds{1}^{#1}}{d_{#1}} \otimes \Tr_{#1}\left[ #2 \right] }
\newcommand{\TrX}[2]{\mathrm{Tr}_{#1}\left[ #2 \right]}
\newcommand{\InProd}[2]{\left\langle #1 \left. ,\, #2 \right. \right\rangle}
\newcommand{\Lbra}[1]{\left( #1 \right|}
\newcommand{\Lket}[1]{\left| #1 \right)}
\newcommand{\OutProd}[2]{\left| #1 \left)\right( #2 \right|}
\newcommand{\GGB}[2]{\sigma^{#1}_{#2}}
\newcommand{\Proj}[2]{\mathcal{P}^{#1}_{#2}}
\newcommand{\CompProj}[2]{\prescript{Q}{}{\mathcal{P}}^{#1}_{#2}}
\newcommand{\ProjOn}[3]{\mathcal{P}^{#1}_{#2}\left[#3\right]}
\newcommand{\MaxMixState}[1]{\left.\left| #1 \right\rangle\right\rangle}
\newcommand{\MaxMixOp}[2]{\left.\left| #1 \right\rangle\right\rangle\left\langle\left\langle #2 \right|\right.}
\newcommand{\Party}[3]{#1^{(#2)}_{#3}}
\newcommand{\Dep}[2]{\prescript{}{#1}{#2}}
\newcommand{\DepPar}[2]{\prescript{}{#1}{\left(#2\right)}}
\newcommand{\PartySet}[2]{\left\{ #1^{(#2)} \right\} }

==> Version 2.0 sent to Quantum/theorems.tex <==
\newtheorem{theo}{Theorem}
\newtheorem{defi}{Definition}
\newtheorem{lemm}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{coro}{Corollary}
